Photodissociation of Cr(CO)$_4$bpy: A non-adiabatic dynamics investigation

Carbonyl complexes of $d^6$ metals with an alpha-diimine ligand exhibit both emission and ligand-selective photodissociation from MLCT states. Studying this photodissociative mechanism is challenging for experimental approaches due to an ultrafast femtosecond timescale and spectral overlap of multiple photoproducts. The photochemistry of a prototypical system Cr(CO)$_4$bpy is investigated with non-adiabatic dynamic simulations. Obtained 86 fs lifetime of the bright $S_3$ state and 13% quantum yield are in good agreement with experimental data. The present simulations suggest a ballistic mechanism of photodissociation, which is irrespective of the occupied electronic state. This is in contrast to the previously established mechanism of competitive intersystem crossing and dissociation. Selectivity of axial photodissociation is shown to be caused by the absence of an avoided crossing in the equatorial direction.

==> preamble2.tex <==
\usepackage[T1]{fontenc}
\usepackage[backend=biber,style=chem-rsc]{biblatex}
\addbibresource{jccbib.bib}

\usepackage[left=0.3in,right=0.3in,bottom=0.7in,top=0.7in]{geometry}
\usepackage{graphicx}
\usepackage[table]{xcolor}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{mathptmx}
\usepackage{array}
\usepackage{longtable}
\usepackage{dcolumn}
\usepackage{textgreek}
\usepackage{indentfirst}
\usepackage{rotating}
\usepackage{placeins}

\usepackage{caption}

\captionsetup{margin=10pt,font=small,labelfont=bf}
\renewcommand{\thefigure}{S\arabic{figure}}
\renewcommand{\thetable}{S\arabic{table}}

\usepackage{booktabs}
\usepackage[para,flushleft]{threeparttable}

\usepackage{romannum}
\AtBeginDocument{\pagenumbering{arabic}}

\usepackage{pgfplots}
\usepackage{pgfplotstable}

\pgfplotstableset{
    x = coord,
    col sep=comma,
    column type={c},
    columns/symmetry/.append style={	string type},
    columns/tran1/.append style={		string type,column type={r<{$\rightarrow$}}},
    columns/tran2/.append style={		string type,column type={>{\hspace{-11.4pt}}l}},
}

\setlength\tabcolsep{6pt}
\setlength\aboverulesep{0pt}
\setlength\belowrulesep{0pt}
\renewcommand{\arraystretch}{0.7}

\heavyrulewidth=0.08em
\lightrulewidth=0.08em
\cmidrulewidth=0.06em
\cmidrulekern=0.6em

\usepackage{hyperref}
\hypersetup{
    hidelinks=true,
    colorlinks=true,
    linkcolor=black,
    citecolor=blue
}
\newcommand{\TheComplex}{Cr(CO)$_4$bpy}
\linespread{2.0}

\setlength\bibitemsep{0pt}
